C3-SL: Circular Convolution-Based Batch-Wise Compression for Communication-Efficient Split Learning

Most existing studies improve the efficiency of Split learning (SL) by compressing the transmitted features. However, most works focus on dimension-wise compression that transforms high-dimensional features into a low-dimensional space. In this paper, we propose circular convolution-based batch-wise compression for SL (C3-SL) to compress multiple features into one single feature. To avoid information loss while merging multiple features, we exploit the quasi-orthogonality of features in high-dimensional space with circular convolution and superposition. To the best of our knowledge, we are the first to explore the potential of batch-wise compression under the SL scenario. Based on the simulation results on CIFAR-10 and CIFAR-100, our method achieves a 16x compression ratio with negligible accuracy drops compared with the vanilla SL. Moreover, C3-SL significantly reduces 1152x memory and 2.25x computation overhead compared to the state-of-the-art dimension-wise compression method.

==> Tables/OverallComp.tex <==
\begin{table}
\caption{Overall Comparison of Computation and Memory Overhead}
\label{table:comp}
\centering

\resizebox{1.0\linewidth}{!}{

   \arrayrulecolor{black}
    \begin{tabular}{!{\color{black}\vrule}c!{\color{black}\vrule}c!{\color{black}\vrule}c!{\color{black}\vrule}c!{\color{black}\vrule}} 
    \hline
    \textbf{Method}                                                           & \textbf{\textit{R}} & \begin{tabular}[c]{@{}c@{}}\textbf{Number of }\\\textbf{Parameters}\end{tabular} & \textbf{FLOPs (x10\textsuperscript{9})}  \\ 
\hline

\multirow{4}{*}{BottleNet++}                                              & 2                  & 9,438,720                     & 4.83                                     \\ 
\cline{2-4}
                                                                          & 4                  & 8,390,656                     & 2.68                                     \\ 
\cline{2-4}
                                                                          & 8                  & 4,195,840                     & \textbf{1.34}                            \\ 
\cline{2-4}
                                                                          & 16                 & 2,098,432                     & \textbf{0.67}                            \\
\hline
\multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Proposed}\\ \textbf{C3-SL}\end{tabular}} & 2                  & \textbf{8,192}                & \textbf{2.15}                            \\ 
\cline{2-4}
                                                                          & 4                  & \textbf{16,384}               & \textbf{2.15}                            \\ 
\cline{2-4}
                                                                          & 8                  & \textbf{32,768}               & 2.15                                     \\ 
\cline{2-4}
                                                                          & 16                 & \textbf{65,536}               & 2.15                                     \\ 
\hline
\end{tabular}
\arrayrulecolor{black}
}

\end{table}


% \usepackage{multirow}
% \usepackage{colortbl}


\begin{table}
\centering

\end{table}


==> Tables/testacc_cifar10.tex <==
\begin{table}[h]
\centering
\vspace{-4mm}
\caption{\textbf{Overall comparison on Cifar-10}}
\vspace{1mm}
\begin{tabular}{c|c|c|c|c} 
\hline
\textbf{Method}                 & \bm{$R$} & \textbf{Accuracy} & \textbf{Number of Parameters} & \textbf{FLOPs (\bm{$\times10^9$})}  \\ 

\hline
\multirow{1}{*}{Vanilla SL~(w/o compression)}    & - & 0.8710        & -           & -  \\ 
\hline
\multirow{6}{*}{BottleNet++}    & 2   & 0.8737   & 9,438,720                     & 4.83                           \\ 
\cline{2-5}
                                & 4   & 0.8736            & 8,390,656                     & 2.68                           \\ 
\cline{2-5}
                                & 8   & 0.8736            & 4,195,840                     & \textbf{1.34}                 \\ 
\cline{2-5}
                                & 16  & 0.8703   & 2,098,432                     & \textbf{0.67}                  \\
\cline{2-5}
                                & 32  & 0.8693   & 1,049,728                     & \textbf{0.34}                  \\
\cline{2-5}
                                & 64  & 0.8690   & 525,376                     & \textbf{0.17}                  \\
\hline
\multirow{6}{*}{\textbf{Proposed C3-SL}} & 2   & 0.8718            & \textbf{8,192}                & \textbf{2.15}                 \\ 
\cline{2-5}
                                & 4   & 0.8710   & \textbf{16,384}               & \textbf{2.15}                \\ 
\cline{2-5}
                                & 8   & 0.8708   & \textbf{32,768}               & 2.15                           \\ 
\cline{2-5}
                                & 16  & 0.8685            & \textbf{65,536}               & 2.15                           \\ 
\cline{2-5}
                                & 32  & 0.8689            & \textbf{131,072}               & 2.15                           \\ 
\cline{2-5}
                                & 64  & 0.8636           & \textbf{262,144}               & 2.15                           \\ 
\hline
\end{tabular}
\vspace{-5mm}
\end{table}

==> Tables/testacc_cifar100.tex <==
\begin{table}[t]
\centering
\vspace{0mm}
\caption{\textbf{Overall comparison on Cifar-100}}
\vspace{1mm}
\begin{tabular}{c|c|c|c|c} 
\hline
\textbf{Method}                 & \bm{$R$} & \textbf{Accuracy} & \textbf{Number of Parameters} & \textbf{FLOPs (\bm{$\times10^9$})}  \\ 
\hline
\multirow{1}{*}{Vanilla SL~(w/o compression)}    & - & 0.6312        & -           & -  \\ 
\hline
\multirow{4}{*}{BottleNet++}    & 2   & 0.6358   & 9,438,720                     & 4.83                           \\ 
\cline{2-5}
                                & 4   & 0.6293            & 8,390,656                     & 2.68                           \\ 
\cline{2-5}
                                & 8   & 0.6265            & 4,195,840                     & \textbf{1.34}                 \\ 
\cline{2-5}
                                & 16  & 0.6255   & 2,098,432                     & \textbf{0.67}                  \\
\hline
\multirow{4}{*}{\textbf{Proposed C3-SL}} & 2   & 0.6343            & \textbf{8,192}                & \textbf{2.15}                 \\ 
\cline{2-5}
                                & 4   & 0.6332   & \textbf{16,384}               & \textbf{2.15}                \\ 
\cline{2-5}
                                & 8   & 0.6280   & \textbf{32,768}               & 2.15                           \\ 
\cline{2-5}
                                & 16  & 0.6229            & \textbf{65,536}               & 2.15                           \\ 
\hline
\end{tabular}
\end{table}

==> Tables/testacc_vgg16.tex <==
\begin{table}[h]
\centering
\vspace{-5mm}
\caption{\textbf{Overall comparison with VGG16 trained on Cifar-10}}
\vspace{1mm}
\begin{tabular}{c|c|c|c|c} 
\hline
\textbf{Method}                 & \bm{$R$} & \textbf{Accuracy} & \textbf{Number of Parameters} & \textbf{FLOPs (\bm{$\times10^8$})}  \\ 
\hline
\multirow{1}{*}{Vanilla SL~(w/o compression)}    & - & 0.8993        & -           & -  \\ 
\hline
\multirow{4}{*}{BottleNet++}    & 2   & 0.9058   & 2,360,064
                     & 12.08                           \\ 
\cline{2-5}
                                & 4   & 0.9041            & 2,098,176
                     & 6.71                           \\ 
\cline{2-5}
                                & 8   & 0.8978            & 1,049,344
                     & \textbf{3.36}                 \\ 
\cline{2-5}
                                & 16  & 0.8961   & 524,928
                     & \textbf{1.68}                  \\
\hline
\multirow{4}{*}{\textbf{Proposed C3-SL}} & 2   & 0.9033            & \textbf{4,096}                & \textbf{5.37}                 \\ 
\cline{2-5}
                                & 4   & 0.8998   & \textbf{8,192}               & \textbf{5.37}                \\ 
\cline{2-5}
                                & 8   & 0.8985   & \textbf{16,384}               & 5.37                           \\ 
\cline{2-5}
                                & 16  & 0.8961            & \textbf{32,768}               & 5.37                           \\ 
\hline
\end{tabular}
\vspace{-7mm}
\end{table}
